Changing-Look AGNs -- I. Tracking the transition on the main sequence of quasars

This paper is the first in a series of preparing and analyzing spectral and other properties for a database of already discovered Changing-Look active galactic nuclei (CL AGNs). Here, we focus on the spectral fitting and analysis of broad emission lines in a sample of 93 CL AGNs collected from the literature with existing SDSS/BOSS/eBOSS spectroscopy where the H$\beta$ emission line profile does not completely disappear in any epochs. Additionally, we have gathered older/newer spectral epochs from all the available SDSS data releases to make the database more complete. We use PyQSOFit and perform a homogeneous spectral decomposition of all of our SDSS spectra and tabulate the AGN continuum and emission line properties per epoch per source, chronologically. This further allows us to categorize the sources in our sample as \textit{Turn-On} or \textit{Turn-Off} and subsequently check for repeated occurrences of such phases. We then estimate the black hole mass (M$_{\rm BH}$) and the Eddington ratio (L$_{\rm bol}$/L$_{\rm Edd}$) per epoch per source where the required parameters are available and well-estimated. We realize the movement of the source in the M$_{\rm BH}$ versus L$_{\rm bol}$/L$_{\rm Edd}$ plane allowing us to check for systematic changes in the source's fundamental properties. We then track their transition along the optical plane of the Eigenvector 1 (EV1) schema and categorize sources that either stay within the same Population (A or B) or make an inter-population movement as a function of spectral epoch. We also test the Balmer decrement (H$\alpha$/H$\beta$) of a subset of our sample of CL AGNs as a function of time and AGN luminosity.

==> table1_observational_lim.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{lscape}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longrotatetable}
\begin{longtable}{llccccccr}
\caption{Details of the sources in our sample (full table can be found in the electronic version)}
\label{tab:table-observe}\\
\hline
Sample & Source & \multicolumn{1}{c}{Plate} & \multicolumn{1}{c}{MJD} & \multicolumn{1}{c}{Fiber} & \multicolumn{1}{c}{RA} & \multicolumn{1}{c}{Dec} & \multicolumn{1}{c}{z} & \multicolumn{1}{c}{Ref.} \\ \hline
\endfirsthead
%
\multicolumn{9}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\hline
Sample & Source & \multicolumn{1}{c}{Plate} & \multicolumn{1}{c}{MJD} & \multicolumn{1}{c}{Fiber} & \multicolumn{1}{c}{RA} & \multicolumn{1}{c}{Dec} & \multicolumn{1}{c}{z} & \multicolumn{1}{c}{Ref.} \\ \hline
\endhead
%
\hline
\endfoot
%
\endlastfoot
%
\citet{lamassa2015} & SDSSJ015957.6+003310 & 403 & 51871 & 549 & 29.990148 & 0.55291729 & 0.31182525 & legacy \\
 &  & 3609 & 55201 & 524 & 29.990161 & 0.55290301 & 0.3120502 & commissioning \\
 &  & 9384$^{\dagger{}}$ & 58080 & 605 & 29.990187 & 0.55289999 & 0.3121399 & ELG\_SGC \\ \hline

 
\citet{Runnoe2016} & SDSSJ101152.98+544206.4 & 945 & 52652 & 22 & 152.97075 & 54.701776 & 0.2463892 & legacy \\
 &  & 8181 & 57073 & 827 & 152.97078 & 54.701786 & 0.24651496 & eboss \\ \hline

 
\citet{macleod2016} & SDSSJ022556.0+003026 & 705 & 52200 & 342 & 36.483662 & 0.50746587 & 0.50387114 & southern \\
 &  & 1508 & 52944 & 556 & 36.483654 & 0.507422 & 0.50425416 & southern \\
 &  & 3615 & 55179 & 641 & 36.483664 & 0.50742591 & 0.5040848 & commissioning \\
... & ... & ... & ... & ... & ... & ... & ... & ... \\ 
... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
\end{longtable}
\footnotesize{{\sc Notes.} Columns are as follows: (1) Reference paper. (2) SDSS identifier for the source. (3) SDSS Plate ID. (4) SDSS date of observation (in modified Julian day). (5) SDSS Fiber ID. (6) right ascension (RA) in degrees. (7) declination in degrees. (8) redshift. (9) original source used to collect the spectrum. Sources marked with $\dagger{}$ in column (3) have either wrong redshift, noisy spectrum with no broad \hb{} detected, or problems with the FITS file. Such sources are removed from further analysis.}
\end{longrotatetable}

==> table2_Lmono_EW_lim.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{lscape}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longrotatetable}
\begin{longtable}{llccccccr}
\caption{Spectral parameters for the sample using {\sc PyQSOFit} - I (full table can be found in the electronic version)}
\label{tab:table-pyqsofit-ew}\\
\hline
Sample & Source & \multicolumn{1}{c}{MJD} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}log L$_{3000}$\\ {[}erg/s{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}log L$_{5100}$\\ {[}erg/s{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}log L$_{6000}$\\ {[}erg/s{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}EW(MgII)\\ {[}\AA{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}EW(H$\beta$)\\ {[}\AA{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}EW(H$\alpha$)\\ {[}\AA{]}\end{tabular}} \\ \hline
\endfirsthead
%
\multicolumn{9}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\hline
Sample & Source & \multicolumn{1}{c}{MJD} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}log L$_{3000}$\\ {[}erg/s{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}log L$_{5100}$\\ {[}erg/s{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}log L$_{6000}$\\ {[}erg/s{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}EW(MgII)\\ {[}\AA{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}EW(H$\beta$)\\ {[}\AA{]}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}EW(H$\alpha$)\\ {[}\AA{]}\end{tabular}} \\ \hline
\endhead
%
\hline
\endfoot
%
\endlastfoot
%
\citet{lamassa2015} & SDSSJ015957.6+003310 & 51871 & 44.09$\pm$0.01 & 44.18$\pm$0.01 & 44.14$\pm$0.02 & -- & 75.65$\pm$4.63 & 109.55$\pm$12.22 \\
 &  & 55201 & 43.59$\pm$0.00 & 43.92$\pm$0.00 & 43.95$\pm$0.01 & 173.30$\pm$48.02 & 71.91$\pm$3.90 & 28.18$\pm$2.34 \\ \hline

 
\citet{Runnoe2016} & SDSSJ101152.98+544206.4 & 52652 & -- & 43.75$\pm$0.00 & 43.54$\pm$0.01 & -- & 155.16$\pm$8.21 & 825.03$\pm$10.38 \\
 &  & 57073 & -- & 43.50$\pm$0.00 & 43.40$\pm$0.02 & -- & 29.33$\pm$15.54 & 33.35$\pm$3.69 \\ \hline

 
\citet{macleod2016} & SDSSJ022556.0+003026 & 52200 & 44.09$\pm$0.00 & 44.26$\pm$0.01 & 44.24$\pm$0.02 & 99.62$\pm$25.88 & 18.95$\pm$4.42 & -- \\
 &  & 52944 & 44.35$\pm$0.01 & 44.38$\pm$0.01 & 44.32$\pm$0.02 & 113.59$\pm$13.34 & 35.63$\pm$3.69 & -- \\
 &  & 55179 & 43.55$\pm$0.01 & 44.06$\pm$0.01 & 44.15$\pm$0.02 & 139.68$\pm$23.14 & 66.35$\pm$2.80 & 13.93$\pm$3.35 \\
... & ... & ... & ... & ... & ... & ... & ... & ... \\
... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
\end{longtable}
\footnotesize{{\sc Notes.} Columns are as follows: (1) Reference paper. (2) SDSS identifier for the source. (3) Date of observation (in modified Julian day). (4) AGN continuum luminosity at 3000\AA~. (5) AGN continuum luminosity at 5100\AA~. (6) AGN continuum luminosity at 6000\AA~. (7) Equivalent width (EW) of \mg{}. (8) EW of \hb{}. (9) EW of \ha{}.}
\end{longrotatetable}

==> table3_RFe_MBH_Eddr_delL_lim.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{lscape}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longrotatetable}
\begin{longtable}{llcccccccr}
\caption{Spectral parameters for the sample using {\sc PyQSOFit} - II (full table can be found in the electronic version)}
\label{tab:table-pyqsofit}\\
\hline
Sample & Source & MJD & \begin{tabular}[c]{@{}c@{}}FWHM(H$\beta_{\rm broad}$)\\ {[}km s$^{-1}${]}\end{tabular} & R$_{\rm FeII}$ & \begin{tabular}[c]{@{}c@{}}log L$_{5100}$\\ {[}erg s$^{-1}${]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}log L$_{\rm bol}$\\ {[}erg s$^{-1}${]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}log M$_{\rm BH}$\\ {[}M$_{\odot}${]}\end{tabular} & log $\lambda_{\rm Edd}$ & \begin{tabular}[c]{@{}c@{}}$\Delta$L$_{5100}$\\ {[}10$^{44}$ erg s$^{-1}${]}\end{tabular} \\ \hline\\
\endfirsthead
%
\multicolumn{10}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\hline
Sample & Source & MJD & \begin{tabular}[c]{@{}c@{}}FWHM(H$\beta_{\rm broad}$)\\ {[}km s$^{-1}${]}\end{tabular} & R$_{\rm FeII}$ & \begin{tabular}[c]{@{}c@{}}log L$_{5100}$\\ {[}erg s$^{-1}${]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}log L$_{\rm bol}$\\ {[}erg s$^{-1}${]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}log M$_{\rm BH}$\\ {[}M$_{\odot}${]}\end{tabular} & log $\lambda_{\rm Edd}$ & \begin{tabular}[c]{@{}c@{}}$\Delta$L$_{5100}$\\ {[}10$^{44}$ erg s$^{-1}${]}\end{tabular} \\ \hline\\
\endhead
%
\hline
\endfoot
%
\endlastfoot
%
\citet{lamassa2015} & SDSSJ015957.6+003310 & 51871 & 6220$\pm$435 & 0.22$\pm$0.06 & 44.18$\pm$0.01 & 45.15$\pm$0.01 & 8.59$\pm$0.06 & -1.58$\pm$0.07 & 0 \\
 &  & 55201 & 16866$\pm$1114 & 1.06$\pm$0.06 & 43.92$\pm$0.00 & 44.89$\pm$0.00 & 9.32$\pm$0.06 & -2.58$\pm$0.06 & -0.692 \\ \hline

 
\citet{Runnoe2016} & SDSSJ101152.98+544206.4 & 52652 & 2826$\pm$122 & 0.60$\pm$0.04 & 43.75$\pm$0.00 & 44.72$\pm$0.00 & 7.69$\pm$0.00 & -1.11$\pm$0.01 & 0 \\
 &  & 57073 & 17862$\pm$9079 & -- & 43.50$\pm$0.00 & 44.47$\pm$0.00 & 9.16$\pm$0.44 & -2.84$\pm$0.44 & -0.245 \\ \hline

 
\citet{macleod2016} & SDSSJ022556.0+003026 & 52200 & 7181$\pm$3545 & 0.00$\pm$0.06 & 44.26$\pm$0.01 & 45.23$\pm$0.01 & 8.75$\pm$0.43 & -1.67$\pm$0.44 & 0 \\
 &  & 52944 & 7715$\pm$1518 & 0.38$\pm$0.08 & 44.38$\pm$0.01 & 45.35$\pm$0.01 & 8.88$\pm$0.17 & -1.67$\pm$0.18 & 0.605 \\
 &  & 55179 & 16218$\pm$1009 & 1.11$\pm$0.06 & 44.06$\pm$0.01 & 45.03$\pm$0.01 & 9.36$\pm$0.06 & -2.47$\pm$0.06 & -0.667 \\ 
... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\
... & ... & ... & ... & ... & ... & ... & ... & ... & ... \\ \hline
\end{longtable}
\footnotesize{{\sc Notes.} Columns are as follows: (1) Reference paper. (2) SDSS identifier for the source. (3) Date of observation (in modified Julian day). (4) Full-width at half-maximum for the broad-component of \hb{}. (5) the ratio \rfe{}. (6) Optical continuum luminosity at 5100\AA~. (7) Bolometric luminosity. (8) Black hole mass. (9) Eddington ratio. (10) difference between the L$_{5100}$ of the source observed at a given MJD to the first observation of the same source.}
\end{longrotatetable}
